A bag of tricks: Using proper motions of Galactic stars to identify the Hercules ultra-faint dwarf galaxy members

Hercules is the prototype of the ultra-faint dwarf (UFD) galaxies. To date, there are still no firm constraints on its total luminosity, due to the difficulty of disentangling Hercules bona-fide stars from the severe Galactic field contamination. In order to better constrain Hercules properties we aim at removing foreground and background contaminants in the galaxy field using the proper motions of the Milky Way stars and the colour-colour diagram. We have obtained images of Hercules in the rSloan, BBessel and Uspec bands with the Large Binocular Telescope (LBT) and LBC-BIN mode capabilities. The rSloan new data-set combined with data from the LBT archive span a time baseline of about 5 yr, allowing us to measure for the first time proper motions of stars in the Hercules direction. The Uspec data along with existing LBT photometry allowed us to use colour-colour diagram to further remove the field contamination. Thanks to a highly-accurate procedure to derive the rSloan-filter geometric distortion solution for the LBC-red, we were able to measure stellar relative proper motions to a precision of better than 5 mas yr^-1 down to rSloan=22 mag and disentangle a significant fraction (\>90\%) of Milky Way contaminants. We ended up with a sample of 528 sources distributed over a large portion of the galaxy body (0.12 deg^2). Of these sources, 171 turned out to be background galaxies and additional foreground stars, from the analysis of the Uspec - BBessel vs. BBessel - rSloan colour-colour diagram. This leaves us with a sample of 357 likely members of the Hercules UFD. We compared the cleaned colour-magnitude diagram (CMD) with evolutionary models and synthetic CMDs, confirming the presence in Hercules of an old population (t=12\pm 2 Gyr), with a wide spread in metallicity (-3.3\<[Fe/H]\<-1.8).

==> tab2.tex <==
001 & 247.8386 &  12.8540 &  18.92$\pm$0.03 &  18.17$\pm$0.01 &  17.36$\pm$0.02 &   0.06$\pm$0.09 \\
002 & 247.8689 &  12.7897 &  18.14$\pm$0.01 &  18.14$\pm$0.01 &  17.84$\pm$0.02 &   0.02$\pm$0.06 \\
003 & 247.9269 &  12.7312 &  19.81$\pm$0.02 &  18.80$\pm$0.01 &  17.88$\pm$0.01 &   0.03$\pm$0.04 \\
004 & 247.9150 &  12.8006 &  21.59$\pm$0.03 &  19.77$\pm$0.01 &  18.24$\pm$0.01 &   0.03$\pm$0.07 \\
005 & 247.8111 &  12.8634 &  20.30$\pm$0.04 &  19.34$\pm$0.01 &  18.30$\pm$0.01 &   0.02$\pm$0.06 \\
006 & 247.7385 &  12.7891 &  21.88$\pm$0.04 &  19.98$\pm$0.04 &  18.31$\pm$0.04 &   0.03$\pm$0.03 \\
007 & 247.7318 &  12.7109 &  19.98$\pm$0.00 &  19.28$\pm$0.01 &  18.57$\pm$0.01 &   0.01$\pm$0.07 \\
008 & 247.5811 &  12.8411 &  20.04$\pm$0.03 &  19.32$\pm$0.01 &  18.61$\pm$0.01 &   0.04$\pm$0.03 \\
009 & 247.8457 &  12.7467 &  21.82$\pm$0.05 &  20.16$\pm$0.01 &  18.65$\pm$0.01 &   0.02$\pm$0.05 \\
010 & 247.7372 &  13.0069 &       \dots     &  19.74$\pm$0.01 &  18.70$\pm$0.01 &   0.03$\pm$0.07 \\
011 & 247.8491 &  12.7781 &  20.89$\pm$0.02 &  19.80$\pm$0.01 &  18.75$\pm$0.01 &   0.00$\pm$0.04 \\
012 & 247.7472 &  12.7905 &  21.37$\pm$0.01 &  20.09$\pm$0.01 &  18.82$\pm$0.02 &   0.02$\pm$0.05 \\
013 & 247.9674 &  12.7206 &  21.26$\pm$0.04 &  20.16$\pm$0.01 &  19.06$\pm$0.03 &   0.01$\pm$0.07 \\
014 & 247.7839 &  12.8018 &  21.71$\pm$0.01 &  20.39$\pm$0.01 &  19.07$\pm$0.01 &   0.00$\pm$0.03 \\
015 & 247.6467 &  12.8285 &  20.67$\pm$0.02 &  19.90$\pm$0.01 &  19.09$\pm$0.03 &   0.01$\pm$0.05 \\
016 & 247.7051 &  12.8465 &  22.66$\pm$0.04 &  20.71$\pm$0.01 &  19.10$\pm$0.01 &   0.02$\pm$0.03 \\
017 & 247.7627 &  12.8794 &  19.50$\pm$0.02 &  19.42$\pm$0.10 &  19.13$\pm$0.04 &   0.04$\pm$0.08 \\
018 & 247.6855 &  12.8300 &  21.57$\pm$0.09 &  20.35$\pm$0.01 &  19.15$\pm$0.01 &   0.04$\pm$0.04 \\
019 & 247.8523 &  12.6566 &  21.46$\pm$0.02 &  20.28$\pm$0.01 &  19.17$\pm$0.01 &   0.04$\pm$0.04 \\
020 & 247.8741 &  12.7404 &  21.61$\pm$0.05 &  20.40$\pm$0.01 &  19.17$\pm$0.02 &   0.03$\pm$0.04 \\
021 & 247.7527 &  12.8256 &  21.68$\pm$0.06 &  20.46$\pm$0.01 &  19.22$\pm$0.02 &   0.03$\pm$0.06 \\
022 & 247.8087 &  12.7575 &  21.67$\pm$0.02 &  20.45$\pm$0.01 &  19.24$\pm$0.02 &   0.02$\pm$0.05 \\
023 & 247.8544 &  12.7582 &  21.85$\pm$0.06 &  20.61$\pm$0.01 &  19.36$\pm$0.01 &   0.02$\pm$0.04 \\
024 & 247.8953 &  12.7299 &  21.63$\pm$0.04 &  20.52$\pm$0.01 &  19.44$\pm$0.02 &   0.03$\pm$0.05 \\
025 & 247.7437 &  12.8668 &  20.77$\pm$0.02 &  20.12$\pm$0.01 &  19.55$\pm$0.03 &   0.04$\pm$0.06 \\
026 & 247.7707 &  12.7860 &  21.83$\pm$0.13 &  20.69$\pm$0.02 &  19.56$\pm$0.02 &   0.03$\pm$0.04 \\
027 & 247.7588 &  12.7238 &  21.76$\pm$0.05 &  20.67$\pm$0.01 &  19.59$\pm$0.01 &   0.03$\pm$0.05 \\
028 & 247.7854 &  12.7281 &  21.09$\pm$0.03 &  20.37$\pm$0.00 &  19.69$\pm$0.02 &   0.03$\pm$0.06 \\
029 & 247.7535 &  12.8015 &  21.21$\pm$0.03 &  20.48$\pm$0.01 &  19.78$\pm$0.01 &   0.03$\pm$0.03 \\
030 & 247.7844 &  12.8008 &  22.04$\pm$0.04 &  20.95$\pm$0.02 &  19.84$\pm$0.01 &   0.01$\pm$0.03 \\
031 & 247.6666 &  12.8340 &  21.59$\pm$0.03 &  20.75$\pm$0.02 &  19.84$\pm$0.01 &   0.01$\pm$0.06 \\
032 & 247.7601 &  12.8008 &  22.09$\pm$0.07 &  20.97$\pm$0.01 &  19.86$\pm$0.01 &   0.03$\pm$0.04 \\
033 & 247.6449 &  12.8336 &  21.14$\pm$0.23 &  20.55$\pm$0.02 &  19.94$\pm$0.02 &   0.04$\pm$0.05 \\
034 & 247.7688 &  12.7708 &  22.11$\pm$0.07 &  20.98$\pm$0.01 &  19.97$\pm$0.23 &   0.02$\pm$0.04 \\
035 & 247.9543 &  12.6839 &  23.73$\pm$0.07 &  21.65$\pm$0.03 &  20.00$\pm$0.01 &   0.03$\pm$0.06 \\
036 & 247.8412 &  12.6784 &  22.11$\pm$0.03 &  21.10$\pm$0.02 &  20.01$\pm$0.01 &   0.03$\pm$0.06 \\
037 & 247.7821 &  12.8055 &  22.26$\pm$0.05 &  21.17$\pm$0.02 &  20.07$\pm$0.01 &   0.01$\pm$0.03 \\
038 & 247.6914 &  12.7910 &  20.13$\pm$0.01 &  20.20$\pm$0.01 &  20.09$\pm$0.24 &   0.03$\pm$0.06 \\
039 & 247.8137 &  12.7457 &  21.81$\pm$0.06 &  20.90$\pm$0.01 &  20.17$\pm$0.02 &   0.02$\pm$0.04 \\
040 & 247.6736 &  12.6687 &  21.81$\pm$0.05 &  21.00$\pm$0.02 &  20.17$\pm$0.01 &   0.03$\pm$0.06 \\
041 & 247.9094 &  12.7435 &  22.12$\pm$0.13 &  21.11$\pm$0.01 &  20.17$\pm$0.01 &   0.03$\pm$0.04 \\
042 & 247.8473 &  12.9893 &       \dots     &  20.76$\pm$0.02 &  20.17$\pm$0.01 &   0.02$\pm$0.05 \\
043 & 247.7257 &  12.8837 &  21.58$\pm$0.10 &  20.89$\pm$0.02 &  20.21$\pm$0.02 &   0.04$\pm$0.06 \\
044 & 247.7934 &  12.9839 &  21.51$\pm$0.04 &  20.81$\pm$0.02 &  20.25$\pm$0.02 &   0.03$\pm$0.04 \\
045 & 247.9235 &  12.6706 &  21.57$\pm$0.01 &  20.88$\pm$0.02 &  20.26$\pm$0.01 &   0.02$\pm$0.06 \\
046 & 247.7556 &  12.7634 &  21.53$\pm$0.02 &  20.88$\pm$0.01 &  20.34$\pm$0.01 &   0.02$\pm$0.04 \\
047 & 247.6054 &  12.8182 &  22.19$\pm$0.06 &  21.28$\pm$0.02 &  20.34$\pm$0.02 &   0.02$\pm$0.07 \\
048 & 247.8128 &  12.6395 &  22.48$\pm$0.11 &  21.41$\pm$0.03 &  20.36$\pm$0.01 &   0.02$\pm$0.06 \\
049 & 247.8027 &  12.8122 &  21.96$\pm$0.10 &  21.11$\pm$0.02 &  20.41$\pm$0.01 &   0.01$\pm$0.04 \\
050 & 247.6186 &  12.7534 &  23.73$\pm$0.31 &  21.91$\pm$0.04 &  20.42$\pm$0.01 &   0.04$\pm$0.06 \\
051 & 247.7912 &  12.7951 &  22.57$\pm$0.16 &  21.48$\pm$0.01 &  20.42$\pm$0.01 &   0.01$\pm$0.04 \\
052 & 247.7242 &  12.8451 &  21.57$\pm$0.04 &  21.01$\pm$0.02 &  20.45$\pm$0.02 &   0.03$\pm$0.05 \\
053 & 247.7996 &  12.9454 &  21.77$\pm$0.07 &  21.05$\pm$0.02 &  20.46$\pm$0.02 &   0.03$\pm$0.05 \\
054 & 247.7865 &  12.6453 &  21.80$\pm$0.04 &  21.18$\pm$0.02 &  20.50$\pm$0.01 &   0.03$\pm$0.04 \\
055 & 247.6416 &  12.7907 &  21.96$\pm$0.54 &  21.32$\pm$0.02 &  20.52$\pm$0.01 &   0.01$\pm$0.05 \\
056 & 247.7776 &  12.7622 &  21.88$\pm$0.11 &  20.70$\pm$0.01 &  20.52$\pm$0.02 &   0.04$\pm$0.02 \\
057 & 247.7042 &  12.8004 &  22.34$\pm$0.06 &  21.40$\pm$0.01 &  20.53$\pm$0.01 &   0.02$\pm$0.04 \\
058 & 247.7119 &  12.8004 &  22.68$\pm$0.09 &  21.63$\pm$0.03 &  20.57$\pm$0.01 &   0.02$\pm$0.04 \\
059 & 247.8154 &  12.7064 &  21.81$\pm$0.09 &  21.17$\pm$0.01 &  20.59$\pm$0.01 &   0.02$\pm$0.06 \\
060 & 247.7033 &  12.8255 &  22.80$\pm$0.10 &  21.66$\pm$0.02 &  20.61$\pm$0.01 &   0.02$\pm$0.03 \\
061 & 247.7620 &  12.7635 &  22.17$\pm$0.02 &  21.11$\pm$0.13 &  20.65$\pm$0.10 &   0.03$\pm$0.05 \\
062 & 247.9226 &  12.8419 &  22.01$\pm$0.01 &  21.23$\pm$0.03 &  20.65$\pm$0.02 &   0.03$\pm$0.07 \\
063 & 247.9854 &  12.7199 &  21.97$\pm$0.07 &  21.27$\pm$0.03 &  20.73$\pm$0.02 &   0.02$\pm$0.07 \\
064 & 247.8125 &  12.7922 &  22.79$\pm$0.12 &  21.75$\pm$0.02 &  20.77$\pm$0.01 &   0.01$\pm$0.03 \\
065 & 247.9269 &  12.6710 &  22.15$\pm$0.07 &  21.46$\pm$0.01 &  20.79$\pm$0.03 &   0.01$\pm$0.07 \\
066 & 247.7229 &  13.0168 &       \dots     &  21.27$\pm$0.01 &  20.88$\pm$0.32 &   0.03$\pm$0.07 \\
067 & 247.7396 &  12.7738 &  22.34$\pm$0.11 &  21.49$\pm$0.03 &  20.93$\pm$0.01 &   0.03$\pm$0.05 \\
068 & 247.8092 &  12.6314 &  22.84$\pm$0.18 &  21.94$\pm$0.05 &  20.95$\pm$0.02 &   0.04$\pm$0.08 \\
069 & 247.6981 &  12.8307 &  23.88$\pm$0.28 &  22.35$\pm$0.09 &  20.98$\pm$0.01 &   0.05$\pm$0.04 \\
070 & 247.8352 &  12.7175 &  22.35$\pm$0.07 &  21.62$\pm$0.03 &  20.99$\pm$0.02 &   0.05$\pm$0.08 \\
071 & 247.7652 &  12.8790 &  22.47$\pm$0.08 &  21.65$\pm$0.01 &  21.02$\pm$0.02 &   0.02$\pm$0.08 \\
072 & 247.7422 &  12.7826 &  23.06$\pm$0.13 &  21.96$\pm$0.05 &  21.02$\pm$0.29 &   0.01$\pm$0.03 \\
073 & 247.7588 &  12.7928 &  21.93$\pm$0.06 &  21.28$\pm$0.36 &  21.03$\pm$0.32 &   0.02$\pm$0.06 \\
074 & 247.8169 &  12.7712 &  23.13$\pm$0.16 &  22.00$\pm$0.03 &  21.04$\pm$0.03 &   0.02$\pm$0.04 \\
075 & 247.8169 &  12.7742 &  22.94$\pm$0.07 &  22.06$\pm$0.04 &  21.06$\pm$0.01 &   0.02$\pm$0.04 \\
076 & 247.7028 &  12.7921 &  22.93$\pm$0.12 &  22.01$\pm$0.03 &  21.10$\pm$0.02 &   0.00$\pm$0.06 \\
077 & 247.8362 &  12.7822 &  23.09$\pm$0.17 &  22.09$\pm$0.03 &  21.10$\pm$0.02 &   0.03$\pm$0.07 \\
078 & 247.9473 &  12.8595 &  22.62$\pm$0.13 &  21.85$\pm$0.02 &  21.13$\pm$0.03 &   0.03$\pm$0.09 \\
079 & 247.9581 &  12.7259 &  22.66$\pm$0.03 &  21.90$\pm$0.02 &  21.14$\pm$0.03 &   0.03$\pm$0.06 \\
080 & 247.7486 &  12.7924 &  23.60$\pm$0.20 &  22.30$\pm$0.05 &  21.14$\pm$0.02 &   0.03$\pm$0.07 \\
081 & 247.8812 &  12.7141 &  22.70$\pm$0.09 &  21.90$\pm$0.03 &  21.15$\pm$0.02 &   0.04$\pm$0.06 \\
082 & 247.7556 &  12.7871 &  23.93$\pm$1.41 &  22.10$\pm$0.02 &  21.15$\pm$0.01 &   0.02$\pm$0.07 \\
083 & 247.7177 &  12.8201 &  22.38$\pm$0.12 &  21.32$\pm$0.02 &  21.16$\pm$0.12 &   0.04$\pm$0.06 \\
084 & 247.7112 &  12.8085 &  22.73$\pm$0.07 &  21.69$\pm$0.01 &  21.16$\pm$0.02 &   0.02$\pm$0.06 \\
085 & 247.7241 &  12.7777 &  23.30$\pm$0.07 &  22.16$\pm$0.03 &  21.16$\pm$0.01 &   0.04$\pm$0.06 \\
086 & 247.7797 &  12.7747 &  22.90$\pm$0.24 &  22.16$\pm$0.06 &  21.17$\pm$0.02 &   0.03$\pm$0.06 \\
087 & 247.6020 &  12.7941 &  22.70$\pm$0.03 &  21.92$\pm$0.03 &  21.18$\pm$0.02 &   0.05$\pm$0.05 \\
088 & 247.9419 &  12.8555 &  22.61$\pm$0.05 &  21.78$\pm$0.03 &  21.19$\pm$0.02 &   0.03$\pm$0.06 \\
089 & 247.6090 &  12.7788 &       \dots     &  22.88$\pm$0.07 &  21.23$\pm$0.02 &   0.03$\pm$0.07 \\
090 & 247.9340 &  12.7178 &  22.56$\pm$0.19 &  21.78$\pm$0.01 &  21.23$\pm$0.01 &   0.03$\pm$0.06 \\
091 & 247.6728 &  12.7570 &  24.14$\pm$0.56 &  22.63$\pm$0.08 &  21.23$\pm$0.02 &   0.03$\pm$0.08 \\
092 & 247.8580 &  12.8394 &  22.84$\pm$0.06 &  22.00$\pm$0.02 &  21.24$\pm$0.01 &   0.05$\pm$0.04 \\
093 & 247.7294 &  12.8708 &  22.71$\pm$0.16 &  21.94$\pm$0.04 &  21.24$\pm$0.02 &   0.04$\pm$0.08 \\
094 & 247.7181 &  12.9075 &  23.27$\pm$0.34 &  22.23$\pm$0.03 &  21.25$\pm$0.02 &   0.03$\pm$0.06 \\
095 & 247.7263 &  12.7982 &  22.51$\pm$0.10 &  21.79$\pm$0.02 &  21.27$\pm$0.02 &   0.03$\pm$0.05 \\
096 & 247.7495 &  12.7699 &  23.05$\pm$0.24 &  22.14$\pm$0.04 &  21.28$\pm$0.01 &   0.01$\pm$0.07 \\
097 & 247.8630 &  12.7380 &  23.06$\pm$0.14 &  21.80$\pm$0.32 &  21.32$\pm$0.15 &   0.01$\pm$0.07 \\
098 & 247.6890 &  12.8180 &  23.47$\pm$0.31 &  22.27$\pm$0.04 &  21.34$\pm$0.02 &   0.04$\pm$0.04 \\
099 & 247.9418 &  12.7001 &  22.79$\pm$0.19 &  21.94$\pm$0.02 &  21.35$\pm$0.02 &   0.04$\pm$0.09 \\
100 & 247.7182 &  12.8334 &  22.89$\pm$0.06 &  21.82$\pm$0.03 &  21.36$\pm$0.10 &   0.04$\pm$0.08 \\
101 & 247.8483 &  12.7575 &  22.95$\pm$0.28 &  21.59$\pm$0.05 &  21.39$\pm$0.04 &   0.02$\pm$0.07 \\
102 & 247.6174 &  12.7741 &  23.18$\pm$0.40 &  22.15$\pm$0.04 &  21.39$\pm$0.02 &   0.03$\pm$0.08 \\
103 & 247.7293 &  12.8383 &  23.20$\pm$0.15 &  22.33$\pm$0.04 &  21.40$\pm$0.03 &   0.02$\pm$0.05 \\
104 & 247.5909 &  12.8105 &  22.81$\pm$0.24 &  22.16$\pm$0.06 &  21.41$\pm$0.02 &   0.04$\pm$0.09 \\
105 & 247.7288 &  12.7845 &  22.81$\pm$0.04 &  21.71$\pm$0.13 &  21.41$\pm$0.27 &   0.02$\pm$0.05 \\
106 & 247.9456 &  12.8015 &  22.82$\pm$0.08 &  22.03$\pm$0.03 &  21.42$\pm$0.02 &   0.02$\pm$0.08 \\
107 & 247.6754 &  12.7964 &  23.32$\pm$0.20 &  22.34$\pm$0.07 &  21.43$\pm$0.23 &   0.03$\pm$0.07 \\
108 & 247.7338 &  12.8082 &  23.05$\pm$0.18 &  21.85$\pm$0.11 &  21.46$\pm$0.02 &   0.00$\pm$0.07 \\
109 & 247.6827 &  12.7981 &  22.68$\pm$0.13 &  21.49$\pm$0.02 &  21.47$\pm$0.03 &   0.05$\pm$0.07 \\
110 & 247.7043 &  12.9091 &       \dots     &  22.63$\pm$0.10 &  21.48$\pm$0.03 &   0.05$\pm$0.07 \\
111 & 247.7484 &  12.7832 &  23.46$\pm$1.80 &  21.55$\pm$0.02 &  21.49$\pm$0.04 &   0.04$\pm$0.05 \\
112 & 247.7236 &  12.8064 &  22.70$\pm$0.26 &  22.08$\pm$0.04 &  21.49$\pm$0.03 &   0.04$\pm$0.03 \\
113 & 247.9624 &  12.7486 &  22.82$\pm$0.14 &  21.55$\pm$0.02 &  21.50$\pm$0.03 &   0.04$\pm$0.10 \\
114 & 247.7606 &  12.8298 &       \dots     &  21.54$\pm$0.01 &  21.50$\pm$0.02 &   0.04$\pm$0.07 \\
115 & 247.9129 &  12.7831 &  22.99$\pm$0.17 &  22.21$\pm$0.03 &  21.51$\pm$0.02 &   0.02$\pm$0.08 \\
116 & 247.9394 &  12.7288 &  23.83$\pm$0.08 &  22.63$\pm$0.06 &  21.51$\pm$0.02 &   0.03$\pm$0.09 \\
117 & 247.7754 &  12.7951 &  22.86$\pm$0.09 &  21.55$\pm$0.02 &  21.52$\pm$0.02 &   0.01$\pm$0.07 \\
118 & 247.8611 &  12.7930 &  22.83$\pm$0.16 &  21.58$\pm$0.02 &  21.52$\pm$0.03 &   0.02$\pm$0.05 \\
119 & 247.6634 &  12.7573 &  23.09$\pm$0.13 &  22.27$\pm$0.07 &  21.53$\pm$0.02 &   0.03$\pm$0.08 \\
120 & 247.9701 &  12.7467 &  22.88$\pm$0.21 &  21.54$\pm$0.01 &  21.54$\pm$0.02 &   0.03$\pm$0.10 \\
121 & 247.8661 &  12.8130 &  22.81$\pm$0.09 &  21.57$\pm$0.03 &  21.54$\pm$0.03 &   0.03$\pm$0.07 \\
122 & 247.7876 &  12.7669 &  23.55$\pm$0.09 &  22.55$\pm$0.07 &  21.58$\pm$0.02 &   0.03$\pm$0.06 \\
123 & 247.7567 &  12.7861 &  23.70$\pm$0.19 &  22.52$\pm$0.06 &  21.59$\pm$0.03 &   0.01$\pm$0.04 \\
124 & 247.7828 &  12.7933 &  22.73$\pm$0.28 &  21.63$\pm$0.01 &  21.59$\pm$0.03 &   0.00$\pm$0.06 \\
125 & 247.7977 &  12.7786 &  23.59$\pm$0.36 &  22.53$\pm$0.05 &  21.60$\pm$0.03 &   0.02$\pm$0.08 \\
126 & 247.7731 &  12.6091 &  23.34$\pm$0.25 &  22.48$\pm$0.05 &  21.63$\pm$0.01 &   0.06$\pm$0.10 \\
127 & 247.7689 &  12.8833 &  23.30$\pm$0.15 &  22.40$\pm$0.04 &  21.65$\pm$0.01 &   0.02$\pm$0.09 \\
128 & 247.9166 &  12.7174 &  22.88$\pm$0.06 &  22.15$\pm$0.02 &  21.66$\pm$0.03 &   0.02$\pm$0.06 \\
129 & 247.6087 &  12.7651 &  23.37$\pm$0.23 &  22.42$\pm$0.06 &  21.68$\pm$0.02 &   0.03$\pm$0.06 \\
130 & 247.7902 &  12.7777 &  23.97$\pm$0.47 &  22.62$\pm$0.08 &  21.68$\pm$0.03 &   0.02$\pm$0.05 \\
131 & 247.7779 &  12.8204 &  23.60$\pm$0.58 &  22.64$\pm$0.06 &  21.71$\pm$0.02 &   0.05$\pm$0.09 \\
132 & 247.9474 &  12.7185 &  24.06$\pm$0.14 &  22.77$\pm$0.10 &  21.71$\pm$0.02 &   0.06$\pm$0.09 \\
133 & 247.7413 &  12.7853 &  23.82$\pm$0.37 &  22.64$\pm$0.06 &  21.73$\pm$0.07 &   0.04$\pm$0.10 \\
134 & 247.8121 &  12.8013 &  23.69$\pm$0.29 &  22.68$\pm$0.06 &  21.74$\pm$0.02 &   0.02$\pm$0.08 \\
135 & 247.6006 &  12.7788 &  23.32$\pm$0.56 &  22.66$\pm$0.06 &  21.75$\pm$0.04 &   0.03$\pm$0.09 \\
136 & 247.9370 &  12.8344 &  23.08$\pm$0.11 &  22.28$\pm$0.04 &  21.76$\pm$0.04 &   0.06$\pm$0.09 \\
137 & 247.8300 &  12.7149 &  23.46$\pm$0.09 &  22.60$\pm$0.06 &  21.77$\pm$0.03 &   0.06$\pm$0.10 \\
138 & 248.0375 &  12.7549 &  23.63$\pm$0.15 &  22.66$\pm$0.06 &  21.82$\pm$0.05 &   0.07$\pm$0.07 \\
139 & 247.7540 &  12.9255 &       \dots     &  23.25$\pm$0.10 &  21.83$\pm$0.03 &   0.05$\pm$0.04 \\
140 & 248.0352 &  12.6928 &  24.21$\pm$0.13 &  22.90$\pm$0.03 &  21.83$\pm$0.03 &   0.06$\pm$0.12 \\
141 & 247.7476 &  12.7533 &  23.56$\pm$0.16 &  22.72$\pm$0.07 &  21.84$\pm$0.04 &   0.04$\pm$0.10 \\
142 & 247.9179 &  12.8062 &  23.57$\pm$0.09 &  22.63$\pm$0.07 &  21.85$\pm$0.02 &   0.07$\pm$0.09 \\
143 & 247.8064 &  12.7895 &  23.48$\pm$0.30 &  22.49$\pm$0.08 &  21.85$\pm$0.04 &   0.06$\pm$0.07 \\
144 & 247.7737 &  12.8972 &  24.22$\pm$0.21 &  22.92$\pm$0.12 &  21.85$\pm$0.06 &   0.07$\pm$0.10 \\
145 & 247.7918 &  12.6571 &  23.97$\pm$0.23 &  23.01$\pm$0.16 &  21.86$\pm$0.05 &   0.06$\pm$0.05 \\
146 & 247.6979 &  12.8174 &  23.65$\pm$0.12 &  22.75$\pm$0.08 &  21.87$\pm$0.03 &   0.05$\pm$0.09 \\
147 & 247.8670 &  12.8070 &       \dots     &  23.63$\pm$0.17 &  21.89$\pm$0.04 &   0.07$\pm$0.11 \\
148 & 247.6037 &  12.8806 &       \dots     &  22.84$\pm$0.07 &  21.89$\pm$0.03 &   0.06$\pm$0.07 \\
149 & 247.7949 &  12.6732 &  23.85$\pm$0.24 &  22.77$\pm$0.07 &  21.91$\pm$0.04 &   0.06$\pm$0.10 \\
150 & 247.6574 &  12.7917 &  23.16$\pm$0.02 &  22.63$\pm$0.09 &  21.95$\pm$0.08 &   0.06$\pm$0.15 \\
151 & 247.8115 &  12.9712 &  23.62$\pm$0.08 &  22.83$\pm$0.11 &  21.97$\pm$0.05 &   0.08$\pm$0.12 \\
152 & 247.7514 &  12.7786 &  23.87$\pm$0.46 &  22.83$\pm$0.07 &  21.97$\pm$0.02 &   0.01$\pm$0.10 \\
153 & 247.8549 &  12.8513 &  24.52$\pm$1.49 &  22.99$\pm$0.12 &  21.98$\pm$0.06 &   0.03$\pm$0.09 \\
154 & 247.7020 &  12.8427 &  24.51$\pm$0.39 &  23.41$\pm$0.15 &  21.98$\pm$0.05 &   0.01$\pm$0.08 \\
155 & 247.8027 &  12.8757 &  23.64$\pm$0.21 &  22.63$\pm$0.03 &  21.99$\pm$0.07 &   0.04$\pm$0.10 \\
156 & 247.9402 &  12.7242 &  23.42$\pm$0.28 &  22.73$\pm$0.12 &  22.00$\pm$0.07 &   0.07$\pm$0.12 \\
157 & 247.6933 &  12.7365 &  23.96$\pm$0.17 &  22.94$\pm$0.11 &  22.00$\pm$0.06 &   0.05$\pm$0.11 \\
158 & 247.7515 &  12.8117 &  24.31$\pm$0.40 &  22.93$\pm$0.12 &  22.01$\pm$0.08 &   0.01$\pm$0.08 \\
159 & 247.7178 &  12.8035 &  23.57$\pm$0.16 &  22.55$\pm$0.06 &  22.02$\pm$0.05 &   0.06$\pm$0.07 \\
160 & 247.6391 &  12.8217 &  23.88$\pm$0.25 &  22.88$\pm$0.06 &  22.02$\pm$0.05 &   0.08$\pm$0.10 \\
161 & 247.9752 &  12.7280 &  24.00$\pm$0.16 &  22.96$\pm$0.07 &  22.03$\pm$0.03 &   0.05$\pm$0.08 \\
162 & 247.6062 &  12.8463 &  23.75$\pm$0.63 &  22.82$\pm$0.06 &  22.04$\pm$0.05 &   0.07$\pm$0.12 \\
163 & 247.7811 &  12.7460 &  24.16$\pm$0.21 &  23.00$\pm$0.13 &  22.05$\pm$0.03 &   0.08$\pm$0.11 \\
164 & 247.8059 &  12.8690 &  23.39$\pm$0.34 &  22.67$\pm$0.09 &  22.05$\pm$0.04 &   0.07$\pm$0.12 \\
165 & 247.6568 &  12.8314 &       \dots     &  23.80$\pm$0.14 &  22.06$\pm$0.07 &   0.02$\pm$0.15 \\
166 & 247.9953 &  12.7492 &       \dots     &  23.27$\pm$0.24 &  22.11$\pm$0.05 &   0.03$\pm$0.05 \\
167 & 247.5798 &  12.8913 &       \dots     &  23.88$\pm$0.19 &  22.11$\pm$0.08 &   0.02$\pm$0.11 \\
168 & 247.9370 &  12.7805 &  23.76$\pm$0.30 &  22.92$\pm$0.05 &  22.12$\pm$0.06 &   0.02$\pm$0.12 \\
169 & 247.9120 &  12.8021 &  23.60$\pm$0.04 &  22.85$\pm$0.11 &  22.13$\pm$0.07 &   0.02$\pm$0.14 \\
170 & 247.8175 &  12.9857 &  23.46$\pm$0.03 &  22.73$\pm$0.05 &  22.14$\pm$0.06 &   0.05$\pm$0.10 \\
171 & 247.7160 &  12.7798 &  23.26$\pm$0.07 &  22.07$\pm$0.04 &  22.16$\pm$0.05 &   0.04$\pm$0.11 \\
172 & 247.9680 &  12.7755 &  23.86$\pm$0.22 &  23.03$\pm$0.14 &  22.16$\pm$0.08 &   0.06$\pm$0.08 \\
173 & 247.6855 &  12.8187 &  22.88$\pm$0.12 &  22.02$\pm$0.02 &  22.17$\pm$0.05 &   0.06$\pm$0.10 \\
174 & 247.8061 &  12.7446 &  24.06$\pm$0.20 &  23.14$\pm$0.17 &  22.19$\pm$0.13 &   0.06$\pm$0.13 \\
175 & 247.8512 &  12.7536 &  24.26$\pm$0.24 &  23.12$\pm$0.13 &  22.19$\pm$0.05 &   0.07$\pm$0.08 \\
176 & 247.7370 &  12.8099 &       \dots     &  23.67$\pm$0.16 &  22.20$\pm$0.09 &   0.03$\pm$0.15 \\
177 & 247.7190 &  13.0274 &       \dots     &  23.17$\pm$0.08 &  22.21$\pm$0.18 &   0.07$\pm$0.05 \\
178 & 247.8767 &  12.6163 &       \dots     &  23.75$\pm$0.17 &  22.21$\pm$0.07 &   0.09$\pm$0.15 \\
179 & 247.8615 &  12.8527 &  24.38$\pm$0.43 &  23.10$\pm$0.07 &  22.24$\pm$0.05 &   0.04$\pm$0.11 \\
180 & 247.7728 &  12.6367 &  23.74$\pm$0.20 &  23.12$\pm$0.16 &  22.24$\pm$0.10 &   0.09$\pm$0.17 \\
181 & 247.7776 &  12.9897 &  23.33$\pm$0.14 &  22.89$\pm$0.13 &  22.25$\pm$0.05 &   0.04$\pm$0.11 \\
182 & 247.7955 &  12.8763 &  23.77$\pm$0.21 &  22.96$\pm$0.08 &  22.25$\pm$0.06 &   0.03$\pm$0.11 \\
183 & 247.8357 &  12.8705 &       \dots     &  23.78$\pm$0.26 &  22.26$\pm$0.07 &   0.10$\pm$0.13 \\
184 & 247.7955 &  12.7855 &  24.12$\pm$0.28 &  23.24$\pm$0.16 &  22.27$\pm$0.07 &   0.02$\pm$0.10 \\
185 & 247.9405 &  12.7502 &  23.91$\pm$0.25 &  23.00$\pm$0.15 &  22.27$\pm$0.08 &   0.09$\pm$0.14 \\
186 & 247.8320 &  12.7804 &       \dots     &  23.20$\pm$0.14 &  22.27$\pm$0.04 &   0.04$\pm$0.16 \\
187 & 247.8544 &  12.8012 &  24.62$\pm$0.06 &  24.01$\pm$0.17 &  22.28$\pm$0.26 &   0.03$\pm$0.15 \\
188 & 247.8768 &  12.8053 &  24.04$\pm$0.41 &  22.97$\pm$0.08 &  22.29$\pm$0.04 &   0.05$\pm$0.12 \\
189 & 247.7626 &  12.8584 &       \dots     &  23.99$\pm$0.30 &  22.29$\pm$0.06 &   0.09$\pm$0.15 \\
190 & 247.7159 &  12.9096 &  24.34$\pm$0.17 &  23.39$\pm$0.13 &  22.29$\pm$0.10 &   0.10$\pm$0.14 \\
191 & 247.6899 &  12.7738 &  24.07$\pm$0.18 &  23.32$\pm$0.16 &  22.30$\pm$0.05 &   0.02$\pm$0.14 \\
192 & 247.6548 &  12.8138 &       \dots     &  23.71$\pm$0.18 &  22.30$\pm$0.09 &   0.05$\pm$0.10 \\
193 & 247.7254 &  12.8950 &       \dots     &  23.46$\pm$0.17 &  22.30$\pm$0.05 &   0.05$\pm$0.16 \\
194 & 247.6955 &  12.7356 &       \dots     &  23.85$\pm$0.21 &  22.30$\pm$0.05 &   0.02$\pm$0.09 \\
195 & 247.7803 &  12.9329 &  24.08$\pm$0.33 &  23.02$\pm$0.12 &  22.33$\pm$0.06 &   0.11$\pm$0.09 \\
196 & 247.7426 &  12.6165 &  24.59$\pm$0.34 &  23.44$\pm$0.11 &  22.34$\pm$0.10 &   0.07$\pm$0.15 \\
197 & 247.8178 &  12.6623 &       \dots     &  23.54$\pm$0.18 &  22.34$\pm$0.11 &   0.10$\pm$0.16 \\
198 & 247.6787 &  12.8556 &  24.05$\pm$0.12 &  23.00$\pm$0.11 &  22.34$\pm$0.09 &   0.05$\pm$0.10 \\
199 & 247.9332 &  12.6326 &       \dots     &  24.07$\pm$0.29 &  22.35$\pm$0.10 &   0.09$\pm$0.10 \\
200 & 247.8995 &  12.7307 &  24.55$\pm$0.05 &  23.11$\pm$0.12 &  22.35$\pm$0.07 &   0.07$\pm$0.18 \\
201 & 247.7450 &  12.7728 &  23.98$\pm$0.36 &  23.26$\pm$0.11 &  22.36$\pm$0.07 &   0.03$\pm$0.11 \\
202 & 247.7703 &  12.7867 &  24.79$\pm$0.28 &  23.37$\pm$0.14 &  22.37$\pm$0.05 &   0.04$\pm$0.11 \\
203 & 247.7284 &  12.8788 &       \dots     &  23.30$\pm$0.18 &  22.37$\pm$0.08 &   0.05$\pm$0.12 \\
204 & 247.8288 &  12.7844 &  24.25$\pm$0.36 &  23.36$\pm$0.19 &  22.38$\pm$0.09 &   0.01$\pm$0.14 \\
205 & 247.8119 &  12.6353 &  25.12$\pm$0.38 &  23.89$\pm$0.26 &  22.38$\pm$0.07 &   0.10$\pm$0.16 \\
206 & 247.7637 &  12.7773 &  24.33$\pm$0.40 &  23.37$\pm$0.14 &  22.41$\pm$0.09 &   0.05$\pm$0.15 \\
207 & 247.7198 &  12.7098 &       \dots     &  23.66$\pm$0.18 &  22.41$\pm$0.09 &   0.11$\pm$0.15 \\
208 & 247.7451 &  12.8027 &  24.03$\pm$0.48 &  23.25$\pm$0.15 &  22.42$\pm$0.09 &   0.07$\pm$0.15 \\
209 & 247.9140 &  12.7076 &       \dots     &  23.96$\pm$0.26 &  22.42$\pm$0.05 &   0.06$\pm$0.15 \\
210 & 247.6395 &  12.7380 &       \dots     &  24.02$\pm$0.17 &  22.42$\pm$0.09 &   0.03$\pm$0.14 \\
211 & 247.8989 &  12.8353 &       \dots     &  23.55$\pm$0.18 &  22.43$\pm$0.07 &   0.08$\pm$0.09 \\
212 & 247.7081 &  12.7005 &       \dots     &  24.20$\pm$0.30 &  22.46$\pm$0.07 &   0.12$\pm$0.16 \\
213 & 247.8708 &  12.7597 &  24.43$\pm$0.26 &  23.32$\pm$0.16 &  22.46$\pm$0.08 &   0.08$\pm$0.08 \\
214 & 247.8729 &  12.8164 &       \dots     &  23.34$\pm$0.12 &  22.46$\pm$0.09 &   0.07$\pm$0.12 \\
215 & 247.8626 &  12.6832 &       \dots     &  23.99$\pm$0.25 &  22.47$\pm$0.06 &   0.12$\pm$0.15 \\
216 & 247.7896 &  12.6505 &  24.19$\pm$0.49 &  23.23$\pm$0.14 &  22.47$\pm$0.07 &   0.05$\pm$0.16 \\
217 & 247.6827 &  12.7777 &       \dots     &  24.16$\pm$0.21 &  22.47$\pm$0.12 &   0.03$\pm$0.14 \\
218 & 247.6393 &  12.7891 &       \dots     &  23.50$\pm$0.18 &  22.47$\pm$0.06 &   0.01$\pm$0.13 \\
219 & 247.7202 &  12.8546 &       \dots     &  23.75$\pm$0.09 &  22.48$\pm$0.10 &   0.03$\pm$0.14 \\
220 & 247.6906 &  12.7713 &       \dots     &  23.47$\pm$0.21 &  22.49$\pm$0.09 &   0.01$\pm$0.15 \\
221 & 247.7819 &  12.7893 &  24.52$\pm$0.58 &  23.44$\pm$0.22 &  22.50$\pm$0.07 &   0.00$\pm$0.15 \\
222 & 247.7670 &  12.9053 &  24.66$\pm$0.72 &  23.46$\pm$0.19 &  22.52$\pm$0.12 &   0.06$\pm$0.12 \\
223 & 247.7284 &  12.8385 &       \dots     &  24.06$\pm$0.20 &  22.52$\pm$0.14 &   0.09$\pm$0.09 \\
224 & 247.6896 &  12.8925 &       \dots     &  23.56$\pm$0.08 &  22.54$\pm$0.06 &   0.10$\pm$0.13 \\
225 & 247.7612 &  12.7499 &  24.71$\pm$0.29 &  23.48$\pm$0.15 &  22.54$\pm$0.10 &   0.07$\pm$0.10 \\
226 & 247.7547 &  12.7504 &  24.62$\pm$0.41 &  23.41$\pm$0.16 &  22.55$\pm$0.11 &   0.11$\pm$0.16 \\
227 & 247.8416 &  12.7312 &       \dots     &  24.34$\pm$0.19 &  22.55$\pm$0.18 &   0.13$\pm$0.17 \\
228 & 247.5601 &  12.8146 &       \dots     &  23.85$\pm$0.20 &  22.55$\pm$0.06 &   0.06$\pm$0.18 \\
229 & 247.8040 &  12.7404 &  24.28$\pm$0.04 &  23.46$\pm$0.14 &  22.56$\pm$0.09 &   0.05$\pm$0.13 \\
230 & 247.8123 &  12.8273 &  24.29$\pm$0.89 &  23.40$\pm$0.15 &  22.57$\pm$0.12 &   0.12$\pm$0.15 \\
231 & 247.9555 &  12.6360 &       \dots     &  24.20$\pm$0.18 &  22.57$\pm$0.08 &   0.09$\pm$0.23 \\
232 & 247.9234 &  12.7617 &       \dots     &  23.59$\pm$0.16 &  22.59$\pm$0.06 &   0.05$\pm$0.12 \\
233 & 247.7666 &  12.7793 &  24.56$\pm$0.41 &  23.49$\pm$0.14 &  22.59$\pm$0.14 &   0.08$\pm$0.13 \\
234 & 247.8006 &  12.8340 &  24.54$\pm$0.70 &  23.64$\pm$0.29 &  22.60$\pm$0.28 &   0.16$\pm$0.25 \\
235 & 247.8067 &  12.7457 &  24.86$\pm$0.53 &  23.69$\pm$0.22 &  22.60$\pm$0.13 &   0.08$\pm$0.18 \\
236 & 247.8733 &  12.8947 &       \dots     &  23.28$\pm$0.10 &  22.61$\pm$0.11 &   0.03$\pm$0.09 \\
237 & 247.8131 &  12.6454 &  24.64$\pm$0.28 &  23.93$\pm$0.20 &  22.61$\pm$0.08 &   0.16$\pm$0.25 \\
238 & 247.8863 &  12.7912 &  24.65$\pm$0.04 &  23.52$\pm$0.16 &  22.62$\pm$0.08 &   0.03$\pm$0.16 \\
239 & 247.7598 &  12.7883 &       \dots     &  23.50$\pm$0.16 &  22.63$\pm$0.18 &   0.15$\pm$0.20 \\
240 & 247.9014 &  12.8007 &       \dots     &  23.44$\pm$0.13 &  22.64$\pm$0.15 &   0.09$\pm$0.17 \\
241 & 247.7477 &  12.7635 &  22.91$\pm$0.07 &  22.69$\pm$0.07 &  22.64$\pm$0.13 &   0.10$\pm$0.11 \\
242 & 247.8807 &  12.8848 &  23.47$\pm$0.28 &  23.07$\pm$0.11 &  22.64$\pm$0.09 &   0.13$\pm$0.20 \\
243 & 247.8837 &  12.7311 &  23.87$\pm$0.20 &  23.41$\pm$0.15 &  22.64$\pm$0.08 &   0.10$\pm$0.17 \\
244 & 247.8115 &  12.7775 &  24.50$\pm$0.65 &  23.56$\pm$0.20 &  22.65$\pm$0.17 &   0.02$\pm$0.16 \\
245 & 247.9168 &  12.8726 &       \dots     &  23.67$\pm$0.20 &  22.66$\pm$0.12 &   0.00$\pm$0.13 \\
246 & 247.9608 &  12.7748 &  23.83$\pm$0.59 &  22.65$\pm$0.08 &  22.66$\pm$0.10 &   0.03$\pm$0.13 \\
247 & 247.6561 &  12.7948 &       \dots     &  24.03$\pm$0.21 &  22.69$\pm$0.11 &   0.14$\pm$0.15 \\
248 & 247.8391 &  12.7939 &  24.32$\pm$0.25 &  23.70$\pm$0.20 &  22.70$\pm$0.10 &   0.05$\pm$0.13 \\
249 & 247.8187 &  12.8755 &       \dots     &  23.46$\pm$0.13 &  22.70$\pm$0.08 &   0.10$\pm$0.14 \\
250 & 247.6299 &  12.7991 &  24.45$\pm$0.28 &  23.68$\pm$0.22 &  22.71$\pm$0.12 &   0.11$\pm$0.15 \\
251 & 247.8283 &  12.6772 &       \dots     &  24.31$\pm$0.29 &  22.73$\pm$0.21 &   0.18$\pm$0.13 \\
252 & 247.8899 &  12.7428 &       \dots     &  23.93$\pm$0.18 &  22.73$\pm$0.11 &   0.05$\pm$0.19 \\
253 & 247.8650 &  12.7889 &  24.48$\pm$0.09 &  23.61$\pm$0.18 &  22.73$\pm$0.12 &   0.05$\pm$0.15 \\
254 & 247.8878 &  12.7446 &  24.46$\pm$0.40 &  23.43$\pm$0.18 &  22.74$\pm$0.14 &   0.05$\pm$0.16 \\
255 & 247.8489 &  12.6549 &       \dots     &  23.49$\pm$0.13 &  22.74$\pm$0.17 &   0.13$\pm$0.19 \\
256 & 247.7161 &  12.9903 &       \dots     &  23.19$\pm$0.09 &  22.75$\pm$0.26 &   0.19$\pm$0.22 \\
257 & 247.9965 &  12.7556 &       \dots     &  24.13$\pm$0.20 &  22.75$\pm$0.13 &   0.14$\pm$0.35 \\
258 & 247.7300 &  12.8208 &       \dots     &  23.93$\pm$0.18 &  22.76$\pm$0.11 &   0.00$\pm$0.10 \\
259 & 247.6060 &  12.7611 &  24.14$\pm$0.37 &  23.53$\pm$0.15 &  22.76$\pm$0.10 &   0.14$\pm$0.21 \\
260 & 247.7752 &  12.6458 &       \dots     &  24.22$\pm$0.30 &  22.76$\pm$0.15 &   0.12$\pm$0.19 \\
261 & 247.5914 &  12.8857 &       \dots     &  24.12$\pm$0.28 &  22.76$\pm$0.11 &   0.09$\pm$0.18 \\
262 & 247.8129 &  12.7819 &       \dots     &  23.73$\pm$0.18 &  22.76$\pm$0.15 &   0.04$\pm$0.16 \\
263 & 247.6918 &  12.7747 &  24.11$\pm$0.28 &  23.87$\pm$0.12 &  22.77$\pm$0.31 &   0.06$\pm$0.32 \\
264 & 247.8487 &  12.7402 &  24.44$\pm$0.49 &  23.83$\pm$0.12 &  22.77$\pm$0.06 &   0.11$\pm$0.26 \\
265 & 247.6976 &  12.8946 &       \dots     &  23.77$\pm$0.15 &  22.77$\pm$0.10 &   0.15$\pm$0.08 \\
266 & 247.7202 &  12.7596 &  24.49$\pm$0.05 &  23.41$\pm$0.12 &  22.77$\pm$0.12 &   0.09$\pm$0.14 \\
267 & 247.9790 &  12.7744 &       \dots     &  24.27$\pm$0.28 &  22.77$\pm$0.11 &   0.12$\pm$0.26 \\
268 & 247.7941 &  12.7737 &  24.29$\pm$0.22 &  23.70$\pm$0.17 &  22.78$\pm$0.17 &   0.05$\pm$0.19 \\
269 & 247.8121 &  12.7575 &  24.75$\pm$0.21 &  23.64$\pm$0.19 &  22.78$\pm$0.15 &   0.04$\pm$0.19 \\
270 & 247.7151 &  12.8926 &  23.82$\pm$0.28 &  23.70$\pm$0.21 &  22.79$\pm$0.38 &   0.19$\pm$0.28 \\
271 & 247.8091 &  12.7276 &  24.89$\pm$0.18 &  24.01$\pm$0.20 &  22.79$\pm$0.11 &   0.10$\pm$0.16 \\
272 & 247.7359 &  12.8293 &  24.54$\pm$0.29 &  23.58$\pm$0.09 &  22.80$\pm$0.14 &   0.02$\pm$0.23 \\
273 & 247.9108 &  12.7229 &       \dots     &  23.83$\pm$0.24 &  22.81$\pm$0.12 &   0.12$\pm$0.14 \\
274 & 247.7898 &  12.7769 &  24.53$\pm$0.44 &  23.71$\pm$0.22 &  22.81$\pm$0.14 &   0.14$\pm$0.28 \\
275 & 247.7021 &  12.8343 &  24.54$\pm$0.63 &  23.95$\pm$0.24 &  22.81$\pm$0.36 &   0.09$\pm$0.37 \\
276 & 248.0061 &  12.7325 &  24.26$\pm$0.40 &  23.53$\pm$0.20 &  22.82$\pm$0.09 &   0.16$\pm$0.16 \\
277 & 247.8552 &  12.7183 &  24.51$\pm$0.64 &  23.84$\pm$0.28 &  22.82$\pm$0.13 &   0.08$\pm$0.16 \\
278 & 247.7811 &  12.6228 &       \dots     &  24.15$\pm$0.34 &  22.82$\pm$0.19 &   0.12$\pm$0.21 \\
279 & 247.6330 &  12.6808 &  23.93$\pm$0.07 &  23.74$\pm$0.17 &  22.83$\pm$0.13 &   0.18$\pm$0.23 \\
280 & 247.6804 &  12.7454 &       \dots     &  24.32$\pm$0.16 &  22.83$\pm$0.12 &   0.07$\pm$0.29 \\
281 & 247.6280 &  12.7136 &       \dots     &  24.07$\pm$0.27 &  22.84$\pm$0.18 &   0.03$\pm$0.33 \\
282 & 247.6776 &  12.6935 &       \dots     &  23.86$\pm$0.17 &  22.84$\pm$0.15 &   0.19$\pm$0.32 \\
283 & 247.6804 &  12.7454 &       \dots     &  24.32$\pm$0.16 &  22.85$\pm$0.12 &   0.07$\pm$0.29 \\
284 & 247.6095 &  12.6494 &       \dots     &  23.93$\pm$0.24 &  22.87$\pm$0.18 &   0.13$\pm$0.17 \\
285 & 247.7545 &  12.7859 &       \dots     &  23.80$\pm$0.17 &  22.87$\pm$0.15 &   0.12$\pm$0.19 \\
286 & 247.7591 &  12.8393 &       \dots     &  24.30$\pm$0.21 &  22.88$\pm$0.15 &   0.13$\pm$0.20 \\
287 & 247.8533 &  12.7770 &  24.43$\pm$0.59 &  24.07$\pm$0.23 &  22.89$\pm$0.33 &   0.13$\pm$0.24 \\
288 & 247.6923 &  12.8551 &       \dots     &  24.39$\pm$0.43 &  22.89$\pm$0.21 &   0.08$\pm$0.33 \\
289 & 247.8169 &  12.8768 &       \dots     &  23.90$\pm$0.18 &  22.89$\pm$0.25 &   0.08$\pm$0.12 \\
290 & 247.6566 &  12.8457 &  25.14$\pm$0.97 &  23.70$\pm$0.18 &  22.90$\pm$0.15 &   0.04$\pm$0.17 \\
291 & 247.8996 &  12.7138 &       \dots     &  23.90$\pm$0.20 &  22.90$\pm$0.21 &   0.10$\pm$0.22 \\
292 & 247.7775 &  12.7087 &  23.69$\pm$0.45 &  23.33$\pm$0.08 &  22.90$\pm$0.16 &   0.17$\pm$0.42 \\
293 & 248.0084 &  12.6703 &  24.33$\pm$0.01 &  23.58$\pm$0.18 &  22.90$\pm$0.18 &   0.19$\pm$0.29 \\
294 & 247.8407 &  12.7232 &       \dots     &  24.63$\pm$0.35 &  22.91$\pm$0.13 &   0.11$\pm$0.15 \\
295 & 247.9820 &  12.7503 &       \dots     &  24.47$\pm$0.31 &  22.92$\pm$0.08 &   0.13$\pm$0.16 \\
296 & 247.6289 &  12.7239 &       \dots     &  24.01$\pm$0.20 &  22.92$\pm$0.15 &   0.23$\pm$0.38 \\
297 & 247.7595 &  12.8163 &       \dots     &  24.45$\pm$0.10 &  22.92$\pm$0.27 &   0.04$\pm$0.17 \\
298 & 247.7174 &  12.7972 &  24.43$\pm$0.87 &  23.81$\pm$0.16 &  22.92$\pm$0.08 &   0.13$\pm$0.12 \\
299 & 247.6990 &  12.8330 &  23.90$\pm$0.16 &  23.66$\pm$0.15 &  22.92$\pm$0.21 &   0.08$\pm$0.19 \\
300 & 247.9012 &  12.7487 &       \dots     &  23.82$\pm$0.09 &  22.92$\pm$0.31 &   0.07$\pm$0.32 \\
301 & 247.7954 &  12.8364 &       \dots     &  23.46$\pm$0.10 &  22.92$\pm$0.13 &   0.09$\pm$0.10 \\
302 & 247.6862 &  12.8919 &       \dots     &  24.67$\pm$0.41 &  22.92$\pm$0.17 &   0.16$\pm$0.25 \\
303 & 247.6341 &  12.8869 &       \dots     &  24.54$\pm$0.12 &  22.93$\pm$0.13 &   0.09$\pm$0.14 \\
304 & 247.9190 &  12.6923 &       \dots     &  24.69$\pm$0.21 &  22.93$\pm$0.12 &   0.14$\pm$0.27 \\
305 & 247.8662 &  12.8170 &  24.55$\pm$0.66 &  23.72$\pm$0.15 &  22.93$\pm$0.15 &   0.12$\pm$0.14 \\
306 & 247.6729 &  12.6643 &  23.55$\pm$0.49 &  23.45$\pm$0.11 &  22.93$\pm$0.12 &   0.13$\pm$0.40 \\
307 & 247.8038 &  12.7752 &       \dots     &  23.80$\pm$0.17 &  22.94$\pm$0.18 &   0.05$\pm$0.24 \\
308 & 247.9350 &  12.8385 &       \dots     &  24.35$\pm$0.20 &  22.94$\pm$0.26 &   0.21$\pm$0.26 \\
309 & 247.6779 &  12.8599 &       \dots     &  23.77$\pm$0.17 &  22.94$\pm$0.13 &   0.19$\pm$0.19 \\
310 & 247.5959 &  12.7492 &       \dots     &  23.97$\pm$0.25 &  22.95$\pm$0.15 &   0.05$\pm$0.33 \\
311 & 247.7134 &  12.7974 &       \dots     &  24.58$\pm$0.29 &  22.95$\pm$0.22 &   0.08$\pm$0.23 \\
312 & 247.8161 &  12.8786 &       \dots     &  23.38$\pm$0.15 &  22.95$\pm$0.20 &   0.12$\pm$0.20 \\
313 & 247.7897 &  12.8019 &  25.32$\pm$1.10 &  23.81$\pm$0.18 &  22.95$\pm$0.13 &   0.07$\pm$0.20 \\
314 & 247.8304 &  12.7782 &  25.02$\pm$1.24 &  23.45$\pm$0.15 &  22.96$\pm$0.16 &   0.19$\pm$0.15 \\
315 & 247.7736 &  12.7178 &  24.44$\pm$0.25 &  23.92$\pm$0.20 &  22.97$\pm$0.17 &   0.04$\pm$0.43 \\
316 & 247.7195 &  12.9029 &  25.08$\pm$0.28 &  23.98$\pm$0.18 &  22.97$\pm$0.20 &   0.13$\pm$0.25 \\
317 & 247.6709 &  12.7618 &  23.42$\pm$0.19 &  23.48$\pm$0.20 &  22.97$\pm$0.12 &   0.07$\pm$0.22 \\
318 & 247.8591 &  12.7894 &  23.77$\pm$0.23 &  23.83$\pm$0.18 &  22.99$\pm$0.36 &   0.03$\pm$0.30 \\
319 & 247.8261 &  12.8435 &  24.60$\pm$0.35 &  24.16$\pm$0.21 &  22.99$\pm$0.21 &   0.23$\pm$0.40 \\
320 & 247.7229 &  12.9675 &       \dots     &  24.73$\pm$0.27 &  22.99$\pm$0.12 &   0.14$\pm$0.24 \\
321 & 247.8755 &  12.8675 &  24.55$\pm$0.54 &  23.96$\pm$0.17 &  23.01$\pm$0.18 &   0.15$\pm$0.23 \\
322 & 247.6609 &  12.6549 &  22.67$\pm$0.01 &  22.79$\pm$0.09 &  23.01$\pm$0.33 &   0.12$\pm$0.21 \\
323 & 247.8867 &  12.6333 &       \dots     &  24.40$\pm$0.52 &  23.02$\pm$0.23 &   0.22$\pm$0.34 \\
324 & 247.8800 &  12.6967 &  23.75$\pm$0.11 &  23.61$\pm$0.17 &  23.02$\pm$0.31 &   0.21$\pm$0.32 \\
325 & 247.9082 &  12.8228 &       \dots     &  23.39$\pm$0.15 &  23.02$\pm$0.10 &   0.20$\pm$0.20 \\
326 & 247.9345 &  12.8113 &       \dots     &  24.10$\pm$0.26 &  23.02$\pm$0.15 &   0.15$\pm$0.20 \\
327 & 247.8755 &  12.8392 &  23.84$\pm$0.41 &  23.59$\pm$0.20 &  23.03$\pm$0.23 &   0.04$\pm$0.32 \\
328 & 247.7816 &  12.7656 &  24.52$\pm$0.62 &  23.89$\pm$0.17 &  23.03$\pm$0.16 &   0.11$\pm$0.19 \\
329 & 247.8692 &  12.7712 &  23.77$\pm$0.04 &  23.57$\pm$0.21 &  23.03$\pm$0.35 &   0.14$\pm$0.19 \\
330 & 247.8519 &  12.6623 &  24.62$\pm$0.10 &  23.94$\pm$0.19 &  23.04$\pm$0.21 &   0.14$\pm$0.32 \\
331 & 247.8684 &  12.7327 &       \dots     &  24.32$\pm$0.28 &  23.04$\pm$0.32 &   0.13$\pm$0.44 \\
332 & 247.9987 &  12.7524 &       \dots     &  24.61$\pm$0.19 &  23.04$\pm$0.14 &   0.05$\pm$0.19 \\
333 & 247.8871 &  12.7422 &  24.56$\pm$0.11 &  24.10$\pm$0.17 &  23.05$\pm$0.21 &   0.05$\pm$0.32 \\
334 & 247.9108 &  12.8313 &       \dots     &  24.62$\pm$0.38 &  23.06$\pm$0.21 &   0.12$\pm$0.30 \\
335 & 247.9098 &  12.8326 &  24.48$\pm$0.73 &  24.26$\pm$0.27 &  23.06$\pm$0.30 &   0.09$\pm$0.33 \\
336 & 247.8074 &  12.6546 &       \dots     &  24.36$\pm$0.12 &  23.06$\pm$0.18 &   0.17$\pm$0.27 \\
337 & 247.8906 &  12.6426 &       \dots     &  24.04$\pm$0.25 &  23.06$\pm$0.11 &   0.13$\pm$0.24 \\
338 & 247.5909 &  12.7398 &  23.96$\pm$0.65 &  23.85$\pm$0.16 &  23.08$\pm$0.23 &   0.24$\pm$0.39 \\
339 & 247.7482 &  12.8595 &       \dots     &  24.82$\pm$0.10 &  23.08$\pm$0.17 &   0.05$\pm$0.19 \\
340 & 247.7579 &  12.7836 &  23.51$\pm$0.24 &  23.54$\pm$0.30 &  23.09$\pm$0.30 &   0.14$\pm$0.33 \\
341 & 247.8740 &  12.8342 &  24.03$\pm$0.24 &  23.88$\pm$0.36 &  23.09$\pm$0.35 &   0.20$\pm$0.37 \\
342 & 247.9469 &  12.7088 &  23.59$\pm$0.18 &  23.29$\pm$0.13 &  23.10$\pm$0.20 &   0.02$\pm$0.30 \\
343 & 247.9238 &  12.7834 &  24.01$\pm$0.04 &  23.85$\pm$0.30 &  23.10$\pm$0.25 &   0.14$\pm$0.30 \\
344 & 247.9754 &  12.7812 &  24.94$\pm$0.38 &  24.35$\pm$0.18 &  23.10$\pm$0.13 &   0.13$\pm$0.19 \\
345 & 247.6489 &  12.7923 &  24.50$\pm$0.53 &  23.98$\pm$0.22 &  23.11$\pm$0.26 &   0.16$\pm$0.17 \\
346 & 248.0064 &  12.7723 &  24.75$\pm$0.54 &  23.06$\pm$0.07 &  23.11$\pm$0.16 &   0.03$\pm$0.28 \\
347 & 247.8668 &  12.6158 &  23.94$\pm$0.29 &  23.82$\pm$0.17 &  23.12$\pm$0.18 &   0.11$\pm$0.24 \\
348 & 247.7831 &  12.8170 &       \dots     &  24.76$\pm$0.16 &  23.13$\pm$0.18 &   0.08$\pm$0.30 \\
349 & 247.8271 &  12.7968 &  24.52$\pm$0.06 &  23.37$\pm$0.20 &  23.14$\pm$0.29 &   0.24$\pm$0.28 \\
350 & 247.8296 &  12.7049 &  25.29$\pm$0.82 &  23.98$\pm$0.26 &  23.14$\pm$0.23 &   0.17$\pm$0.24 \\
351 & 247.6818 &  12.8122 &  25.17$\pm$0.26 &  23.94$\pm$0.21 &  23.15$\pm$0.20 &   0.05$\pm$0.17 \\
352 & 247.7041 &  12.8165 &  24.46$\pm$0.24 &  23.40$\pm$0.09 &  23.15$\pm$0.18 &   0.08$\pm$0.22 \\
353 & 247.9024 &  12.7908 &       \dots     &  24.10$\pm$0.17 &  23.16$\pm$0.24 &   0.08$\pm$0.28 \\
354 & 247.7545 &  12.8778 &       \dots     &  24.00$\pm$0.28 &  23.17$\pm$0.27 &   0.11$\pm$0.32 \\
355 & 248.0376 &  12.7382 &  23.83$\pm$0.08 &  23.59$\pm$0.17 &  23.17$\pm$0.15 &   0.18$\pm$0.39 \\
356 & 247.8364 &  12.7701 &  24.35$\pm$0.18 &  24.57$\pm$0.41 &  23.17$\pm$0.29 &   0.12$\pm$0.42 \\
357 & 247.6306 &  12.8897 &  24.09$\pm$0.10 &  23.81$\pm$0.05 &  23.18$\pm$0.16 &   0.17$\pm$0.21 \\
358 & 247.7838 &  12.7096 &  24.71$\pm$0.33 &  24.17$\pm$0.17 &  23.19$\pm$0.27 &   0.15$\pm$0.30 \\
359 & 247.9073 &  12.8728 &  24.41$\pm$0.35 &  23.97$\pm$0.20 &  23.19$\pm$0.29 &   0.18$\pm$0.15 \\
360 & 247.8755 &  12.8681 &       \dots     &  24.21$\pm$0.28 &  23.20$\pm$0.26 &   0.05$\pm$0.43 \\
361 & 248.0230 &  12.7434 &       \dots     &  24.44$\pm$0.26 &  23.20$\pm$0.23 &   0.01$\pm$0.12 \\
362 & 247.5762 &  12.7820 &       \dots     &  23.91$\pm$0.21 &  23.20$\pm$0.15 &   0.15$\pm$0.30 \\
363 & 247.6654 &  12.6437 &       \dots     &  24.85$\pm$0.53 &  23.20$\pm$0.12 &   0.12$\pm$0.46 \\
364 & 247.6682 &  12.7804 &  23.88$\pm$0.34 &  23.79$\pm$0.18 &  23.20$\pm$0.18 &   0.12$\pm$0.24 \\
365 & 247.6638 &  12.8653 &  23.85$\pm$0.25 &  23.76$\pm$0.33 &  23.21$\pm$0.31 &   0.17$\pm$0.21 \\
366 & 247.6814 &  12.6768 &  24.77$\pm$0.23 &  24.16$\pm$0.28 &  23.22$\pm$0.26 &   0.26$\pm$0.37 \\
367 & 247.8473 &  12.7450 &  24.13$\pm$0.44 &  24.01$\pm$0.26 &  23.22$\pm$0.24 &   0.22$\pm$0.43 \\
368 & 247.9959 &  12.7467 &       \dots     &  24.28$\pm$0.21 &  23.22$\pm$0.18 &   0.05$\pm$0.19 \\
369 & 247.9107 &  12.7359 &       \dots     &  24.51$\pm$0.17 &  23.22$\pm$0.29 &   0.16$\pm$0.43 \\
370 & 247.8279 &  12.7986 &       \dots     &  24.17$\pm$0.23 &  23.23$\pm$0.23 &   0.14$\pm$0.21 \\
371 & 247.7734 &  12.7905 &       \dots     &  24.46$\pm$0.24 &  23.23$\pm$0.25 &   0.02$\pm$0.26 \\
372 & 247.9031 &  12.6771 &       \dots     &  24.09$\pm$0.17 &  23.23$\pm$0.19 &   0.17$\pm$0.45 \\
373 & 247.5930 &  12.7454 &       \dots     &  24.50$\pm$0.38 &  23.24$\pm$0.19 &   0.14$\pm$0.43 \\
374 & 247.8231 &  12.8164 &  23.22$\pm$0.16 &  23.50$\pm$0.14 &  23.24$\pm$0.27 &   0.19$\pm$0.22 \\
375 & 247.7682 &  12.8957 &       \dots     &  24.48$\pm$0.22 &  23.24$\pm$0.28 &   0.13$\pm$0.31 \\
376 & 247.7078 &  12.8177 &  24.49$\pm$0.58 &  24.32$\pm$0.22 &  23.25$\pm$0.28 &   0.06$\pm$0.33 \\
377 & 247.7777 &  12.7943 &  24.23$\pm$0.30 &  24.01$\pm$0.14 &  23.26$\pm$0.30 &   0.26$\pm$0.37 \\
378 & 247.9054 &  12.8212 &       \dots     &  24.20$\pm$0.14 &  23.27$\pm$0.29 &   0.07$\pm$0.25 \\
379 & 247.8028 &  12.8386 &       \dots     &  24.57$\pm$0.13 &  23.27$\pm$0.23 &   0.12$\pm$0.27 \\
380 & 247.6234 &  12.7172 &       \dots     &  25.00$\pm$0.13 &  23.27$\pm$0.18 &   0.18$\pm$0.19 \\
381 & 247.6890 &  12.6805 &       \dots     &  23.53$\pm$0.19 &  23.28$\pm$0.29 &   0.20$\pm$0.34 \\
382 & 247.6370 &  12.8091 &  24.60$\pm$0.25 &  24.05$\pm$0.08 &  23.28$\pm$0.17 &   0.09$\pm$0.49 \\
383 & 247.8562 &  12.6299 &  23.82$\pm$0.24 &  23.76$\pm$0.23 &  23.28$\pm$0.23 &   0.05$\pm$0.28 \\
384 & 247.6731 &  12.6407 &       \dots     &  24.56$\pm$0.12 &  23.29$\pm$0.22 &   0.23$\pm$0.45 \\
385 & 247.7642 &  12.8235 &  26.15$\pm$3.50 &  24.30$\pm$0.19 &  23.29$\pm$0.20 &   0.25$\pm$0.42 \\
386 & 247.8707 &  12.8155 &       \dots     &  24.47$\pm$0.23 &  23.30$\pm$0.32 &   0.07$\pm$0.37 \\
387 & 247.8641 &  12.7762 &       \dots     &  24.61$\pm$0.24 &  23.30$\pm$0.18 &   0.12$\pm$0.28 \\
388 & 247.6286 &  12.8643 &  23.69$\pm$0.24 &  23.57$\pm$0.08 &  23.31$\pm$0.14 &   0.22$\pm$0.32 \\
389 & 247.7797 &  12.7288 &  24.40$\pm$0.39 &  24.10$\pm$0.22 &  23.31$\pm$0.27 &   0.24$\pm$0.41 \\
390 & 247.6098 &  12.8068 &       \dots     &  24.84$\pm$0.11 &  23.32$\pm$0.28 &   0.17$\pm$0.48 \\
391 & 247.7935 &  12.6190 &  24.41$\pm$0.29 &  24.37$\pm$0.19 &  23.32$\pm$0.20 &   0.06$\pm$0.28 \\
392 & 247.9617 &  12.7384 &       \dots     &  23.52$\pm$0.16 &  23.32$\pm$0.18 &   0.04$\pm$0.22 \\
393 & 247.6987 &  12.7011 &       \dots     &  24.25$\pm$0.16 &  23.32$\pm$0.20 &   0.23$\pm$0.35 \\
394 & 247.7315 &  12.7859 &  24.58$\pm$0.56 &  24.85$\pm$0.39 &  23.33$\pm$0.26 &   0.25$\pm$0.35 \\
395 & 247.7301 &  12.7851 &  24.20$\pm$0.42 &  23.99$\pm$0.27 &  23.33$\pm$0.33 &   0.18$\pm$0.32 \\
396 & 247.6989 &  12.8299 &       \dots     &  24.51$\pm$0.17 &  23.33$\pm$0.22 &   0.19$\pm$0.41 \\
397 & 247.8581 &  12.6846 &  23.93$\pm$0.31 &  23.68$\pm$0.17 &  23.34$\pm$0.21 &   0.28$\pm$0.31 \\
398 & 247.6678 &  12.7995 &       \dots     &  24.53$\pm$0.24 &  23.34$\pm$0.20 &   0.09$\pm$0.21 \\
399 & 247.8477 &  12.6912 &  24.64$\pm$0.43 &  23.89$\pm$0.25 &  23.34$\pm$0.20 &   0.13$\pm$0.21 \\
400 & 247.7854 &  12.8702 &       \dots     &  24.45$\pm$0.19 &  23.35$\pm$0.30 &   0.22$\pm$0.38 \\
401 & 247.7227 &  12.7219 &  24.22$\pm$0.16 &  23.78$\pm$0.13 &  23.35$\pm$0.23 &   0.02$\pm$0.31 \\
402 & 247.7301 &  12.6971 &       \dots     &  24.25$\pm$0.22 &  23.36$\pm$0.30 &   0.23$\pm$0.32 \\
403 & 247.9765 &  12.7767 &  24.09$\pm$0.10 &  24.34$\pm$0.34 &  23.37$\pm$0.18 &   0.08$\pm$0.43 \\
404 & 247.5948 &  12.8129 &  23.98$\pm$0.18 &  23.81$\pm$0.08 &  23.37$\pm$0.17 &   0.15$\pm$0.44 \\
405 & 247.8092 &  12.6558 &  24.94$\pm$0.51 &  23.98$\pm$0.22 &  23.37$\pm$0.24 &   0.16$\pm$0.23 \\
406 & 247.7901 &  12.8283 &  23.65$\pm$0.20 &  23.82$\pm$0.22 &  23.38$\pm$0.21 &   0.02$\pm$0.40 \\
407 & 247.8371 &  12.8119 &  25.01$\pm$0.81 &  24.10$\pm$0.22 &  23.38$\pm$0.23 &   0.09$\pm$0.26 \\
408 & 247.8373 &  12.7687 &       \dots     &  24.31$\pm$0.21 &  23.38$\pm$0.25 &   0.19$\pm$0.25 \\
409 & 247.6580 &  12.7667 &  25.08$\pm$0.45 &  24.13$\pm$0.23 &  23.40$\pm$0.24 &   0.02$\pm$0.16 \\
410 & 247.7311 &  12.7866 &  25.38$\pm$0.90 &  23.54$\pm$0.11 &  23.40$\pm$0.27 &   0.23$\pm$0.37 \\
411 & 247.6297 &  12.8121 &  24.82$\pm$0.38 &  24.06$\pm$0.15 &  23.41$\pm$0.25 &   0.08$\pm$0.13 \\
412 & 247.7084 &  12.6339 &  24.23$\pm$0.05 &  23.95$\pm$0.17 &  23.41$\pm$0.32 &   0.13$\pm$0.31 \\
413 & 247.8192 &  12.8142 &  23.57$\pm$0.22 &  23.46$\pm$0.09 &  23.41$\pm$0.18 &   0.17$\pm$0.24 \\
414 & 247.7134 &  12.7148 &       \dots     &  24.40$\pm$0.28 &  23.42$\pm$0.17 &   0.23$\pm$0.47 \\
415 & 247.6863 &  12.7653 &       \dots     &  23.84$\pm$0.09 &  23.42$\pm$0.11 &   0.23$\pm$0.42 \\
416 & 247.7986 &  12.8692 &       \dots     &  24.27$\pm$0.19 &  23.43$\pm$0.30 &   0.18$\pm$0.39 \\
417 & 247.8122 &  12.8520 &       \dots     &  24.39$\pm$0.24 &  23.43$\pm$0.30 &   0.06$\pm$0.31 \\
418 & 247.6520 &  12.7891 &       \dots     &  24.46$\pm$0.25 &  23.43$\pm$0.25 &   0.16$\pm$0.36 \\
419 & 247.7141 &  12.7365 &       \dots     &  24.54$\pm$0.20 &  23.44$\pm$0.30 &   0.25$\pm$0.50 \\
420 & 247.6935 &  12.8661 &  24.58$\pm$0.94 &  24.04$\pm$0.17 &  23.44$\pm$0.24 &   0.13$\pm$0.33 \\
421 & 247.9724 &  12.6748 &  24.25$\pm$0.79 &  24.04$\pm$0.13 &  23.45$\pm$0.18 &   0.23$\pm$0.24 \\
422 & 247.7484 &  12.8085 &  24.47$\pm$0.19 &  24.19$\pm$0.13 &  23.45$\pm$0.26 &   0.26$\pm$0.48 \\
423 & 248.0173 &  12.7069 &  24.26$\pm$0.36 &  24.23$\pm$0.14 &  23.46$\pm$0.16 &   0.09$\pm$0.46 \\
424 & 247.7529 &  12.7383 &  25.05$\pm$0.13 &  23.43$\pm$0.14 &  23.47$\pm$0.21 &   0.17$\pm$0.26 \\
425 & 247.6645 &  12.6892 &       \dots     &  24.10$\pm$0.17 &  23.48$\pm$0.26 &   0.21$\pm$0.15 \\
426 & 247.7713 &  12.8306 &       \dots     &  24.61$\pm$0.14 &  23.48$\pm$0.22 &   0.15$\pm$0.39 \\
427 & 247.9083 &  12.6740 &       \dots     &  24.91$\pm$0.32 &  23.49$\pm$0.28 &   0.21$\pm$0.51 \\
428 & 248.0383 &  12.7262 &       \dots     &  24.42$\pm$0.29 &  23.50$\pm$0.37 &   0.13$\pm$0.22 \\
429 & 247.7907 &  12.7949 &       \dots     &  24.27$\pm$0.19 &  23.50$\pm$0.19 &   0.22$\pm$0.31 \\
430 & 247.6874 &  12.8144 &       \dots     &  24.96$\pm$0.05 &  23.51$\pm$0.21 &   0.18$\pm$0.19 \\
431 & 247.8984 &  12.7565 &       \dots     &  24.86$\pm$0.17 &  23.52$\pm$0.18 &   0.25$\pm$0.38 \\
432 & 247.9063 &  12.7959 &       \dots     &  24.36$\pm$0.29 &  23.52$\pm$0.20 &   0.23$\pm$0.51 \\
433 & 247.6870 &  12.6549 &       \dots     &  25.32$\pm$0.16 &  23.52$\pm$0.32 &   0.11$\pm$0.28 \\
434 & 247.7191 &  12.7316 &  24.13$\pm$0.54 &  24.27$\pm$0.26 &  23.52$\pm$0.23 &   0.13$\pm$0.36 \\
435 & 247.8376 &  12.6900 &  23.90$\pm$0.16 &  23.80$\pm$0.19 &  23.53$\pm$0.33 &   0.05$\pm$0.42 \\
436 & 247.8936 &  12.7612 &       \dots     &  24.14$\pm$0.25 &  23.53$\pm$0.17 &   0.17$\pm$0.30 \\
437 & 247.9241 &  12.7771 &  24.63$\pm$0.73 &  24.59$\pm$0.21 &  23.53$\pm$0.25 &   0.23$\pm$0.38 \\
438 & 247.7802 &  12.8785 &       \dots     &  24.43$\pm$0.35 &  23.54$\pm$0.27 &   0.27$\pm$0.29 \\
439 & 247.7530 &  12.8161 &  24.93$\pm$0.58 &  24.28$\pm$0.23 &  23.54$\pm$0.26 &   0.23$\pm$0.21 \\
440 & 247.7138 &  12.7934 &       \dots     &  24.30$\pm$0.25 &  23.55$\pm$0.28 &   0.08$\pm$0.24 \\
441 & 247.8473 &  12.7805 &       \dots     &  24.61$\pm$0.31 &  23.55$\pm$0.24 &   0.11$\pm$0.40 \\
442 & 247.7497 &  12.8096 &  24.66$\pm$0.06 &  24.12$\pm$0.26 &  23.56$\pm$0.26 &   0.17$\pm$0.22 \\
443 & 247.6153 &  12.8440 &       \dots     &  24.34$\pm$0.21 &  23.57$\pm$0.24 &   0.04$\pm$0.45 \\
444 & 247.7281 &  12.6257 &  24.34$\pm$0.71 &  24.21$\pm$0.20 &  23.58$\pm$0.25 &   0.22$\pm$0.48 \\
445 & 247.7673 &  12.6906 &  24.30$\pm$0.11 &  24.17$\pm$0.21 &  23.59$\pm$0.25 &   0.17$\pm$0.38 \\
446 & 247.8306 &  12.6491 &  24.05$\pm$0.09 &  23.82$\pm$0.18 &  23.59$\pm$0.30 &   0.06$\pm$0.41 \\
447 & 247.6767 &  12.8652 &  24.35$\pm$0.29 &  23.76$\pm$0.19 &  23.60$\pm$0.17 &   0.22$\pm$0.35 \\
448 & 247.6931 &  12.8202 &       \dots     &  24.30$\pm$0.24 &  23.60$\pm$0.25 &   0.13$\pm$0.28 \\
449 & 247.6052 &  12.8700 &  24.57$\pm$0.82 &  23.79$\pm$0.16 &  23.61$\pm$0.23 &   0.25$\pm$0.51 \\
450 & 247.9289 &  12.7086 &       \dots     &  24.50$\pm$0.31 &  23.61$\pm$0.14 &   0.12$\pm$0.48 \\
451 & 247.8753 &  12.7304 &       \dots     &  25.09$\pm$0.19 &  23.61$\pm$0.29 &   0.05$\pm$0.43 \\
452 & 247.9383 &  12.7425 &       \dots     &  24.02$\pm$0.10 &  23.61$\pm$0.24 &   0.07$\pm$0.33 \\
453 & 247.7695 &  12.7716 &       \dots     &  24.91$\pm$0.30 &  23.61$\pm$0.19 &   0.23$\pm$0.50 \\
454 & 247.6585 &  12.8189 &       \dots     &  24.96$\pm$0.24 &  23.62$\pm$0.16 &   0.04$\pm$0.44 \\
455 & 247.9079 &  12.6705 &       \dots     &  23.90$\pm$0.15 &  23.62$\pm$0.33 &   0.06$\pm$0.19 \\
456 & 247.7497 &  12.7881 &  24.82$\pm$0.80 &  24.43$\pm$0.21 &  23.63$\pm$0.20 &   0.22$\pm$0.28 \\
457 & 247.7955 &  12.7971 &       \dots     &  24.65$\pm$0.32 &  23.63$\pm$0.22 &   0.15$\pm$0.35 \\
458 & 247.8176 &  12.7368 &  25.56$\pm$1.57 &  24.68$\pm$0.29 &  23.63$\pm$0.22 &   0.02$\pm$0.51 \\
459 & 247.8486 &  12.8088 &       \dots     &  24.01$\pm$0.23 &  23.63$\pm$0.20 &   0.18$\pm$0.47 \\
460 & 247.8248 &  12.8403 &       \dots     &  25.10$\pm$0.23 &  23.64$\pm$0.28 &   0.19$\pm$0.45 \\
461 & 247.7935 &  12.7219 &       \dots     &  24.34$\pm$0.26 &  23.64$\pm$0.26 &   0.23$\pm$0.41 \\
462 & 247.9279 &  12.7496 &       \dots     &  24.15$\pm$0.21 &  23.65$\pm$0.19 &   0.06$\pm$0.39 \\
463 & 247.6976 &  12.7733 &       \dots     &  24.95$\pm$0.17 &  23.65$\pm$0.25 &   0.05$\pm$0.24 \\
464 & 247.7808 &  12.7158 &  24.13$\pm$0.44 &  24.19$\pm$0.22 &  23.65$\pm$0.23 &   0.18$\pm$0.33 \\
465 & 247.6977 &  12.8566 &       \dots     &  24.18$\pm$0.23 &  23.66$\pm$0.22 &   0.04$\pm$0.42 \\
466 & 247.7856 &  12.8006 &       \dots     &  24.78$\pm$0.24 &  23.67$\pm$0.24 &   0.04$\pm$0.27 \\
467 & 247.7317 &  12.7667 &  24.52$\pm$0.51 &  24.31$\pm$0.21 &  23.68$\pm$0.29 &   0.14$\pm$0.27 \\
468 & 247.6927 &  12.8380 &       \dots     &  24.56$\pm$0.29 &  23.68$\pm$0.25 &   0.18$\pm$0.26 \\
469 & 247.7483 &  12.7632 &       \dots     &  24.50$\pm$0.32 &  23.69$\pm$0.24 &   0.03$\pm$0.29 \\
470 & 247.7619 &  12.8296 &  24.25$\pm$0.34 &  23.89$\pm$0.10 &  23.69$\pm$0.25 &   0.10$\pm$0.29 \\
471 & 247.7306 &  12.8642 &  24.78$\pm$0.64 &  24.03$\pm$0.20 &  23.70$\pm$0.28 &   0.13$\pm$0.41 \\
472 & 247.8063 &  12.8682 &       \dots     &  24.76$\pm$0.17 &  23.71$\pm$0.22 &   0.16$\pm$0.38 \\
473 & 247.8528 &  12.8742 &       \dots     &  24.08$\pm$0.16 &  23.71$\pm$0.27 &   0.18$\pm$0.44 \\
474 & 247.9274 &  12.7364 &  24.56$\pm$1.29 &  24.14$\pm$0.12 &  23.73$\pm$0.27 &   0.16$\pm$0.25 \\
475 & 247.9325 &  12.7946 &  24.55$\pm$0.42 &  24.26$\pm$0.36 &  23.73$\pm$0.26 &   0.23$\pm$0.47 \\
476 & 247.8862 &  12.6519 &  24.81$\pm$0.40 &  24.35$\pm$0.22 &  23.74$\pm$0.23 &   0.19$\pm$0.42 \\
477 & 247.6286 &  12.8647 &       \dots     &  23.84$\pm$0.13 &  23.74$\pm$0.21 &   0.06$\pm$0.35 \\
478 & 247.6642 &  12.8937 &       \dots     &  24.58$\pm$0.28 &  23.76$\pm$0.31 &   0.04$\pm$0.21 \\
479 & 247.7211 &  12.8084 &  24.61$\pm$0.42 &  24.12$\pm$0.16 &  23.77$\pm$0.27 &   0.04$\pm$0.26 \\
480 & 247.7194 &  12.8186 &       \dots     &  24.75$\pm$0.12 &  23.77$\pm$0.21 &   0.19$\pm$0.41 \\
481 & 247.8674 &  12.8499 &  24.46$\pm$0.44 &  23.97$\pm$0.24 &  23.77$\pm$0.27 &   0.27$\pm$0.31 \\
482 & 247.8825 &  12.7334 &       \dots     &  23.79$\pm$0.13 &  23.78$\pm$0.27 &   0.02$\pm$0.34 \\
483 & 247.7692 &  12.8603 &       \dots     &  25.10$\pm$0.07 &  23.79$\pm$0.25 &   0.08$\pm$0.45 \\
484 & 247.9366 &  12.8219 &  24.12$\pm$0.16 &  24.07$\pm$0.15 &  23.79$\pm$0.23 &   0.12$\pm$0.23 \\
485 & 247.6706 &  12.8158 &       \dots     &  24.06$\pm$0.20 &  23.79$\pm$0.22 &   0.23$\pm$0.28 \\
486 & 247.8203 &  12.8221 &       \dots     &  24.80$\pm$0.12 &  23.82$\pm$0.26 &   0.09$\pm$0.33 \\
487 & 247.8956 &  12.8687 &       \dots     &  24.64$\pm$0.10 &  23.84$\pm$0.26 &   0.05$\pm$0.33 \\
488 & 247.6884 &  12.8095 &  24.62$\pm$0.48 &  24.10$\pm$0.14 &  23.84$\pm$0.28 &   0.12$\pm$0.34 \\
489 & 247.7415 &  12.6522 &       \dots     &  24.45$\pm$0.18 &  23.85$\pm$0.14 &   0.11$\pm$0.46 \\
490 & 247.7873 &  12.8101 &  25.15$\pm$0.08 &  24.42$\pm$0.26 &  23.85$\pm$0.24 &   0.11$\pm$0.34 \\
491 & 247.6959 &  12.6813 &  23.98$\pm$0.05 &  23.90$\pm$0.16 &  23.85$\pm$0.32 &   0.04$\pm$0.27 \\
492 & 247.9285 &  12.7978 &       \dots     &  24.30$\pm$0.21 &  23.86$\pm$0.33 &   0.23$\pm$0.47 \\
493 & 247.8662 &  12.7546 &  25.07$\pm$1.74 &  24.21$\pm$0.25 &  23.86$\pm$0.33 &   0.19$\pm$0.46 \\
494 & 247.8656 &  12.8330 &  24.73$\pm$0.68 &  24.20$\pm$0.21 &  23.87$\pm$0.18 &   0.09$\pm$0.46 \\
495 & 247.6133 &  12.8896 &  23.87$\pm$0.15 &  24.02$\pm$0.17 &  23.88$\pm$0.24 &   0.23$\pm$0.43 \\
496 & 247.7644 &  12.6392 &  24.62$\pm$0.38 &  24.41$\pm$0.20 &  23.89$\pm$0.27 &   0.05$\pm$0.48 \\
497 & 247.8042 &  12.9009 &  24.91$\pm$1.79 &  23.85$\pm$0.20 &  23.89$\pm$0.22 &   0.10$\pm$0.38 \\
498 & 247.8886 &  12.7706 &       \dots     &  24.25$\pm$0.22 &  23.90$\pm$0.28 &   0.03$\pm$0.19 \\
499 & 247.8922 &  12.8911 &       \dots     &  24.04$\pm$0.24 &  23.91$\pm$0.23 &   0.18$\pm$0.44 \\
500 & 247.7766 &  12.8147 &  24.09$\pm$0.17 &  24.09$\pm$0.23 &  23.92$\pm$0.17 &   0.29$\pm$0.45 \\
501 & 247.9730 &  12.7446 &       \dots     &  24.93$\pm$0.20 &  23.92$\pm$0.22 &   0.09$\pm$0.44 \\
502 & 247.6296 &  12.8089 &       \dots     &  24.27$\pm$0.22 &  23.93$\pm$0.23 &   0.21$\pm$0.42 \\
503 & 247.6493 &  12.7391 &       \dots     &  23.84$\pm$0.14 &  23.93$\pm$0.28 &   0.27$\pm$0.29 \\
504 & 247.6956 &  12.6375 &  24.21$\pm$0.50 &  24.09$\pm$0.24 &  23.94$\pm$0.44 &   0.12$\pm$0.36 \\
505 & 247.6721 &  12.8127 &  24.80$\pm$0.60 &  24.48$\pm$0.15 &  23.95$\pm$0.28 &   0.21$\pm$0.38 \\
506 & 247.7517 &  12.6128 &       \dots     &  25.03$\pm$0.09 &  23.96$\pm$0.36 &   0.31$\pm$0.42 \\
507 & 247.9057 &  12.7049 &  24.24$\pm$0.11 &  24.22$\pm$0.22 &  23.97$\pm$0.18 &   0.18$\pm$0.40 \\
508 & 247.7997 &  12.7307 &  24.45$\pm$0.01 &  24.04$\pm$0.11 &  23.98$\pm$0.25 &   0.06$\pm$0.37 \\
509 & 247.7222 &  12.7767 &       \dots     &  23.81$\pm$0.24 &  23.98$\pm$0.31 &   0.20$\pm$0.30 \\
510 & 247.7225 &  12.8961 &  24.77$\pm$0.33 &  24.23$\pm$0.21 &  24.02$\pm$0.26 &   0.27$\pm$0.51 \\
511 & 247.8064 &  12.7663 &       \dots     &  23.87$\pm$0.15 &  24.04$\pm$0.33 &   0.14$\pm$0.29 \\
512 & 247.8556 &  12.7310 &       \dots     &  24.44$\pm$0.24 &  24.09$\pm$0.31 &   0.32$\pm$0.52 \\
513 & 247.6584 &  12.8690 &  24.95$\pm$0.81 &  24.25$\pm$0.11 &  24.09$\pm$0.28 &   0.25$\pm$0.48 \\
514 & 247.8432 &  12.7216 &       \dots     &  24.15$\pm$0.27 &  24.12$\pm$0.25 &   0.05$\pm$0.35 \\
515 & 247.7030 &  12.8106 &  24.85$\pm$0.13 &  24.29$\pm$0.18 &  24.15$\pm$0.24 &   0.24$\pm$0.48 \\
516 & 247.6500 &  12.7644 &       \dots     &  24.48$\pm$0.12 &  24.17$\pm$0.27 &   0.23$\pm$0.46 \\
517 & 247.8951 &  12.7730 &       \dots     &  24.54$\pm$0.30 &  24.20$\pm$0.27 &   0.24$\pm$0.42 \\
518 & 247.7278 &  12.8439 &       \dots     &  25.07$\pm$0.28 &  24.21$\pm$0.21 &   0.18$\pm$0.40 \\
519 & 247.7768 &  12.8061 &       \dots     &  24.37$\pm$0.21 &  24.23$\pm$0.26 &   0.09$\pm$0.44 \\
520 & 247.6551 &  12.7478 &       \dots     &  24.65$\pm$0.15 &  24.23$\pm$0.20 &   0.09$\pm$0.45 \\
521 & 247.7901 &  12.8059 &       \dots     &  24.38$\pm$0.25 &  24.25$\pm$0.31 &   0.16$\pm$0.46 \\
522 & 247.7377 &  12.7451 &  24.23$\pm$0.38 &  24.19$\pm$0.19 &  24.25$\pm$0.40 &   0.30$\pm$0.43 \\
523 & 247.8919 &  12.7432 &       \dots     &  24.53$\pm$0.06 &  24.27$\pm$0.18 &   0.24$\pm$0.45 \\
524 & 247.7172 &  12.7989 &  24.77$\pm$0.38 &  24.70$\pm$0.39 &  24.29$\pm$0.28 &   0.76$\pm$0.51 \\
525 & 247.8143 &  12.8058 &  24.23$\pm$0.23 &  24.54$\pm$0.31 &  24.32$\pm$0.40 &   0.20$\pm$0.24 \\
526 & 247.7700 &  12.7420 &  24.65$\pm$0.24 &  24.63$\pm$0.31 &  24.36$\pm$0.37 &   0.52$\pm$0.47 \\
527 & 247.6952 &  12.7963 &  24.33$\pm$0.23 &  24.66$\pm$0.33 &  24.47$\pm$0.31 &   0.50$\pm$0.48 \\
528 & 247.6628 &  12.8131 &  24.60$\pm$0.16 &  24.58$\pm$0.28 &  24.49$\pm$0.27 &   0.31$\pm$0.53 \\


==> tab3.tex <==
006 &  308205 & 42241$^a$ &  42241$^a$ & \dots &  308205$^a$ & \dots \\
009 & \dots & 41082$^a$ & \dots & \dots & \dots & \dots \\
012 &  308613 & 42149$^a$ &  42149$^a$ & \dots &  308613$^a$ & \dots \\
014 &  308686 & 41743$^a$ &  41743$^a$ & \dots &  308686$^a$ & \dots \\
018 &  308457 & 42795$^a$ &  42795$^a$ & \dots &  308457$^a$ & \dots \\
020 &  309528 & 40789$^a$ &  40789$^a$ & \dots &  309528$^a$ & \dots \\
021 &  308596 & 42096$^a$ &  42096$^a$ & \dots &  308596$^a$ & \dots \\
022 &  309397 & 41460$^a$ &  41460$^a$ & \dots &  309397$^a$ & \dots \\
023 &  309487 & 40993$^a$ &  40993$^a$ & \dots &  309487$^a$ & \dots \\
026 &  308324 & \dots & \dots & \dots & \dots & \dots \\
030 & \dots & 41737$^a$ & \dots & \dots & \dots & \dots \\
032 &  308627 & 42008$^a$ & \dots & \dots &  308627$^a$ & \dots \\
033 & \dots & 43167  & \dots & \dots & \dots & \dots \\
034 &  308674 & 41912$^a$ & \dots & \dots &  308674$^a$ & \dots \\
037 &  308671 & 41758$^a$ & \dots & \dots &  308671$^a$ & \dots \\
039 & \dots & 41401  & \dots & \dots & \dots & \dots \\
041 & \dots & 40435  & \dots & F1-16  & \dots & \dots \\
049 & \dots & 41532  & \dots & \dots & \dots & \dots \\
052 & \dots & \dots & \dots & F2-01  & \dots & \dots \\
057 &  308524 & 42621  & \dots & \dots &  308524$^a$ & \dots \\
060 &  308829 & 42637$^a$ & \dots & \dots &  308829$^a$ & \dots \\
061 & \dots & \dots & \dots & \dots & \dots & V2 \\ 
064 &  309655 & 41423$^a$ & \dots & \dots &  309655$^a$ & \dots \\
073 & \dots & \dots & \dots & F2-07  & \dots & V1$^a$ \\ 
075 &  309663 & \dots & \dots & \dots &  309663$^a$ & \dots \\
083 & \dots & 42484  & \dots & \dots & \dots & V5$^a$ \\ 
084 & \dots & 42550  & \dots & \dots & \dots & \dots \\
085 &  3081382 & \dots & \dots & \dots &  3081382$^a$ & \dots \\
086 &  308327 & \dots & \dots & \dots &  308327$^a$ & \dots \\
097 & \dots & 40911  & \dots & \dots & \dots & V8$^a$ \\ 
098 &  308477 & \dots & \dots & \dots & \dots & \dots \\
100 & \dots & \dots & \dots & \dots & \dots & V6$^a$ \\ 
105 & \dots & 42355  & \dots & \dots & \dots & V3$^a$ \\ 
106 & \dots & \dots & \dots & F1-21  & \dots & \dots \\
108 &  308190 & \dots & \dots & \dots & \dots & V4$^a$ \\ 
111 &  308256 & 42134  & \dots & F2-17  & \dots & \dots \\
113 & \dots & \dots & \dots & F1-10  & \dots & \dots \\
114 & \dots & \dots & \dots & F2-16  & \dots & \dots \\
117 & \dots & \dots & \dots & F2-06  & \dots & \dots \\
118 &  309470 & \dots & \dots & \dots & \dots & \dots \\
120 & \dots & \dots & \dots & F1-09  & \dots & \dots \\
122 &  3081556 & \dots & \dots & \dots &  3081556$^a$ & \dots \\
125 &  308751 & \dots & \dots & \dots & \dots & \dots \\
131 &  3081473 & \dots & \dots & \dots & \dots & \dots \\


